Harpocrates: Privacy-Preserving and Immutable Audit Log for Sensitive Data Operations

The audit log is a crucial component to monitor fine-grained operations over sensitive data (e.g., personal, health) for security inspection and assurance. Since such data operations can be highly sensitive, it is vital to ensure that the audit log achieves not only validity and immutability, but also confidentiality against active threats to standard data regulations (e.g., HIPAA) compliance. Despite its critical needs, state-of-the-art privacy-preserving audit log schemes (e.g., Ghostor (NSDI '20), Calypso (VLDB '19)) do not fully obtain a high level of privacy, integrity, and immutability simultaneously, in which certain information (e.g., user identities) is still leaked in the log. In this paper, we propose Harpocrates, a new privacy-preserving and immutable audit log scheme. Harpocrates permits data store, share, and access operations to be recorded in the audit log without leaking sensitive information (e.g., data identifier, user identity), while permitting the validity of data operations to be publicly verifiable. Harpocrates makes use of blockchain techniques to achieve immutability and avoid a single point of failure, while cryptographic zero-knowledge proofs are harnessed for confidentiality and public verifiability. We analyze the security of our proposed technique and prove that it achieves non-malleability and indistinguishability. We fully implemented Harpocrates and evaluated its performance on a real blockchain system (i.e., Hyperledger Fabric) deployed on a commodity platform (i.e., Amazon EC2). Experimental results demonstrated that Harpocrates is highly scalable and achieves practical performance.

==> motivation.tex <==

Laws such as The Health Insurance Portability and Accountability Act of 1996 (HIPAA) prohibits patient records from being disclosed without the patient's consent or knowledge. 
%
Compliance with HIPAA is a major concern for medical organizations as well as cloud data service providers.
%
A lot of such works \cite{Liu_Access,MedBlock,Medrec,MeDShare,BPDS_globecom2018} do not address the anonymity concerns of patients and employ public blockchains for logging operations on medical data.
Many researchers have leveraged the use of blockchain to record supply chain related operations \cite{Baralla,agri_suuply,poms,iot_supply}.
%
However, transparency in supply chain is not always possible and can be prohibited by law. 
%
The Federal Acquisition Supply Chain Security Act of 2018 (FASCSA) gives power to federal agencies to modify supplier databases and remove information related to orders made by them. \cite{FASCA}
%
Although done due to a matter of national security, this may cause issues for a supplier's bookkeeping and is not the best solution.


==> security_IEEE_tifs.tex <==
\section{Security Analysis}
In this section,
we analyze the security of our proposed scheme.
%
We have the following theorem.
\begin{Theorem}
    \sys~satisfies record non-malleability by \autoref{lnm}.
\end{Theorem}
% \thang{
% \textit{Proof Overview.} We show $\sys$ achieves record non-malleability by defining an adversary who intercepts a record sent to the distributed audit log by an honest user. The adversary then modifies the record and submits it to the audit log for verification.

% However, by highlighting properties of cryptographic primitives used in the system, we show that the adversary's modified record will never be verified by the distributed audit log. Hence, $\sys$ achieves record non-malleability
% }
\begin{proof}
We show that the probability that the adversary can tamper with existing records or create a record activity (e.g., access record without having a proper share record) that he is not authorized to do so is negligible.
%
Consider the following two cases:

    \textbf{Case 1.} Let $Q_\CreateAddress = \{1^\lambda, 1^\lambda, \dotsc\}$ be the queries by $\adv$ to $\CreateAddress$ and $R_\CreateAddress = \{(\addpk^{\provider,1}, \addsk^{\provider,1}), (\addpk^{\provider,2}, \addsk^{\provider,2}), \dotsc\}$ be the response from $\chal$. 
    \sloppy $Q_{\AssignOwner}=\{(\pp,\tokenstore^1,\addsk^{\provider,1},\addpk^{\owner,1}), (\pp,\tokenstore^2,\addsk^{\provider,2},\addpk^{\owner,2}), \dotsc\}$ be the queries created by $\adv$ and $R_{\AssignOwner}=\{(\tokenowner^1, \tx_\assign^1), (\tokenowner^2, \tx_\assign^2), \dotsc\}$ be the response by $\chal$. $\adv$ wins the Log-Entry Non-Malleability game when it outputs a log $ \tx_\own^* $ such that (i) $m^* \neq m$, where $m$ is the message in $\tx_\own \in R_\AssignOwner$;  (ii) $ \mathsf{VerifyLog}(\pp,\tx_\own^*,\set{L}') = 1 $, where $ \set{L}' $ is the state of the audit log preceding $\tx_\own$; (iii) $\sn^*$ revealed in $\tx^*_\own$ is same as in $\tx_\own$.

  We assume that $\adv$ successfully creates an ownership record $\tx_\own^*=(\rt_\store^*, \sigpk^*, \sigma^*,  \sn^*, \cm_\own^*, \h^*, \pi_\own^*, \tokenowner^*)$ with proof instance $ x^* = (\rt_\store^*, \sn^*, \cm_\own^*, h^*)$ and $m^* = x^*||h_\sig^*||\pi_\own^*||\tokenowner^*$. 
    
        Each of the above event captures all the possible modifications $\adv$ makes to $\tx_\store$ to obtain $\tx_\store^*$ such that $m^* \neq m$.
    %
    $E_1$ captures when $m^* \neq m$ but $\pk_\sig^* = \pk_\sig$.
    %
    $E_2$ captures when $m^* \neq m$ but $ \h_\sig^* = \h_\sig$.
    %
    $E_3$ captures when $m^* \neq m$ but $\h^* = \h$.
    %
    $E_3$ captures when $m^* \neq m$. Note that $\sn^* = \sn$ applies to all event as it is the condition of the game.
    
    Let $E_1$ be the event that $\adv$ wins and there exists $\pk_\sig \in R_\AssignOwner$ such that $\pk_\sig^* = \pk_\sig$. %\thang{same pk, but at least one in the signature message should be different}
    
    $E_2:$ $\adv$ wins, $E_1$ does not occur, and there exist $\pk_\sig \in R_\AssignOwner$ such that $h^*_\sig = h_\sig$. %\thang {new $\pk_\sig$, all others do not matter}
    
    $E_3:$ $\adv$ wins, $(E_1, E_2)$ do not occur and  $h^* = \PRF(\addsk^{\provider^*}|| h^*_\sig)$ for some $\addsk^{\provider^*} \in R_\CreateAddress$. %\thang{you need to define Q to store address created by Adv} %\thang{new $h^*$, new pk without CRH with any existing pk, but there is link between them in terms of PRF}.
    
    $E_4:$ $\adv$ wins, $(E_1, E_2, E_3)$ do not occur and  $h^* \ne \PRF(\addsk^{\provider^*}|| h^*_\sig)$ for \textit{all} $\addsk^{\provider^*} \in R_\CreateAddress$. %\thang{completely new $h^*$, $pk^*$}
    
%    $\adv$ wins if each of the following hold independently-
    % Each of the above event captures all the possible modifications $\adv$ makes to $\tx_\own$ to obtain $\tx_\own^*$ such that $\tx_\own^* \neq \tx_\own$.
    % %
    % $E_1$ captures when $\tx_\own^* \neq \tx_\own$ but $\pk_\sig^* = \pk_\sig$.
    % %
    % $E_2$ captures when $\tx_\own^* \neq \tx_\own$ but $ \h_\sig^* = \h_\sig$.
    % %
    % $E_3$ captures when $\tx_\own^* \neq \tx_\own$ but $\h^* = \h$.
    % %
    % $E_4$ captures when $\tx_\own^* \neq \tx_\own$. 
    % %
    % Note that in every event $\sn^* = \sn$ as it is a condition imposed by the game. 
    
    Now we present the intuition to show that each event occurs with negligible probability.
    
    $E_1$ occurs iff $\adv$ can forge a new signature $\sigma^*$ in $\tx^*$ for the message $m^*$ that contain a new serial number $\sn^*$, under the same signing and verification key, which only happens with negligible probability due to the SUF-CMA property of signature scheme.
    
    $E_2$ only occurs iff  $\adv$ can provide a new $\pk^*_\sig$ in $\tx^*$ such that $\CRH(\pk^*_\sig) = \CRH(\pk_\sig)$, which only happens with negligible probability due to the collision-resistant property of $H$
    
    $E_3$ occurs iff $\adv$ can distinguish $\PRF$ from a random function, which happens with negligible probability.
    
    $E_4$ occurs iff $\adv$ can find a collision for the $\PRF$ used to generate $\sn$, which happens only with negligible probability.
    
    \begin{itemize}
        \item We show that $\Pr[E_1] = \negl(\lambda) $. Let $\sigma^*$ be the signature in $\tx^*_\own$ and $\sigma$ be signature in $\tx_\own$ that has $\pk_\sig$. Because  $\pk_\sig = \pk^*_\sig$, both $\sigma^*$ and $\sigma$ are the signatures created from the same public key. Since $\adv$ wins, by definition, there exists $\tx_\own \in R_\AssignOwner $ such that $m^* \ne m$ and $\sn^* = \sn$. To satisfy case this, $\adv$ needs to produce $\sigma^*$ such that $\Sigma.\Verify(\pk_\sig^*, m^*, \sigma^*) = 1$, $m^* \ne m$ and $\pk_\sig = \pk_\sig^*$. However, this happens with negligible probability as it breaks the SUF-CMA property of the underlying signature scheme. Also, as $\sn^* = \sn$, this only happens with negligible probability given that the serial number $\sn = \PRF(\addsk^\owner||\rho)$ is generated by a PRF with a random seed $\rho$. 
        %
       % \thang{I read zcash and actually I see that you can simply follow its proof. Probably to save time, you dont need to give a formal proof here. Maybe lets do this only. You can simply say Event 1 does not happen due to the SUF-CMA of signature scheme. Event 2 does not happen due to the collision-resistant property of H. Event 3 does not happen due to the randomness indintuighsability property of PRF. Event 4 does not happen due to the colision resistant of PRF for sn (note that prf for sn requires collision-resistant, which is different from prf for Event 3. Basically, give the proof sketch or intuition only, no need formal proof}.
        
        \item We show that $\Pr[E_2] = \negl(\lambda) $. 
        Let $h_\sig^*\gets\CRH(\pk_\sig^*)$ be the hash of the signature verification key $\pk_\sig^*$ in $\tx^*_\own$ and $h_\sig=\CRH(\pk_\sig)$ be the hash of the signature verification key $\pk_\sig$ in $\tx_\own$. Since $\adv$ wins, there is a $m^* \ne m$ such that $\h_\sig^*=\h_\sig$. Now when $\pk_\sig^*=\pk_\sig$, it would be handled in $E_1$. When $\pk_\sig^* \ne \pk_\sig$, due to the collision-resistant property of the hash function, $\h_\sig^* = \h_\sig$ cannot hold true.
        
        \item We show that $\Pr[E_3] = \negl(\lambda) $ by contradiction. Assume $\epsilon = \Pr[E_3]$ is non negligible. Now we construct an attacker $\advb$ that distinguishes with a non negligible probability a pseudorandom function $\PRF$ from a random function $\RAND$ by crafting $\tx^\dagger_\own $. $\advb$ follows the same conditions that $\adv$ follows to craft $\tx^*$. To do so, $\advb$ selects a random $(\addpk^{\provider^\dagger}, \addsk^{\provider^\dagger}) \in R_\CreateAddress$. Then, $\advb$ crafts $h^\dagger = \owner^\PRF(\addsk^{\provider^\dagger}||h_\sig^\dagger)$ or $\h^\dagger = \owner^\RAND(\addsk^{\provider^\dagger}||h_\sig^\dagger)$ using either of the two oracles $\owner^\PRF$ or $\owner^\RAND$.
        $\advb$ then invokes $\adv$ which outputs $\tx_\own^*$. Now, according to conditions of $E_3$, $\advb$ outputs 1 (i.e, wins) iff $h^\dagger = \h^*$ where $h^*$ is a part of $\tx_\own^*$ crafted by $\adv$. 
        $\advb$ \textit{aborts and wins} if it outputs $\h^\dagger = \h^*$ \textit{before} $\adv$ outputs $\tx_\own^*$. 
        
        Now, we calculate the probability that $\advb$ wins. Note that $\advb$ wins when it aborts \textit{or} if it outputs 1 and does not abort.  Recall that $\advb$ aborts iff it outputs $\h^\dagger = \h^*$ before $\adv$ outputs a $\h^*$. Then, when $\adv$ finally outputs $h^*$, it would imply that $\pk_\sig^* = \pk_\sig^\dagger$ and $\h_\sig^* = \h_\sig^\dagger$ which does not hold in $E_3$ (when $E_3$ occurs, $E_1$ and $E_2$ don't occur). Hence, $\advb$ aborts with negligible probability. Therefore, to calculate the probability with which $\advb$ wins, it is sufficient to calculate the probability that $\advb$ outputs 1 and does not abort.
        
        Since $\advb$ uses either of the two oracles, we have the following cases -- i) $\h^\dagger$ is created using $\owner^\RAND$.
        If $h^\dagger$ is of one bit length, the probability that $\advb$ wins and does not abort is $\frac{1}{2}$. Since the output is of length $\lvert \h^\dagger \rvert$, the probability that $\advb$ wins and does not abort is ($\frac{1}{2})^{\lvert \h^\dagger \rvert}$, which is negligible. 
        
        ii) $\h^\dagger$ is crafted using $\owner^\PRF$.
        Since $\adv$ performs the experiment independent of $\addsk^{\provider^\dagger}$, probability that $\addsk^{\provider^*} = \addsk^{\provider^\dagger}$ will be $\frac{1}{\lvert R_\CreateAddress \rvert}$. Therefore, the probability that $\advb$ wins and $\advb$ does not aborts is at least $\frac{\epsilon}{\lvert R_\CreateAddress \rvert}$. Since $\epsilon$ is non negligible (by assumption), $\frac{\epsilon}{\lvert R_\CreateAddress \rvert}$ is also non negligible.
        
        Now to calculate the probability that $\advb$ distinguishes between a pseudorandom and a random function, we find the difference in probabilities when $\advb$ wins in i) and ii). Since in ii), $\advb$ wins with a non negligible probability, the difference is non negligible. 
        
        We successfully crafted an attacker $\advb$ that can distinguish between a $\PRF$ and a random function with an overwhelming probability. However, this is a contradiction as a pseudorandom function is indistinguishable from a random function.
        
        \item We show that $\Pr[E_4] = \negl(\lambda) $ by contradiction.  We craft an algorithm $\advb$ which finds collisions in $\PRF$ used to compute $\sn$ with an overwhelming probability. $\advb$ first runs $\adv$ to obtain $\tx_\own^*$. Then, it runs a zero-knowledge extractor $\zkExt$ to obtain a witness $w$. If $w$ is invalid, $\adv$ aborts and returns 0. If $w$ is valid, find $\tx \in R_\AssignOwner$ with $\sn^* = \sn$. If $\addsk^{\provider^*} \ne \addsk^{\provider}$ and $\sn^* = \sn$, $\advb$ found a collision for $\PRF$. 
        
        Now we show that $\addsk^{\provider^*} \ne \addsk^{\provider}$ occurs with overwhelming probability. Since $w$ is valid, $\h^* = \PRF(\addsk^{\provider^*}||h_\sig^*)$. Now, if $\addsk^{\provider^*} = \addsk^\provider$, it contradicts conditions of $E_4$. Therefore, if $E_4$ occurs, $\addsk^{\provider^*} \neq \addsk^\provider$ with overwhelming probability. This implies that $\advb$ always finds a $\tx \in R_\AssignOwner$ such that $\sn^* = \sn$ with an overwhelming probability.
        
        We successfully created an algorithm $\advb$ that finds a collision for $\PRF$ used to create $\sn$ with an overwhelming probability. However, since the $\PRF$ used to create $\sn$ has to be collision-resistant, this is a contradiction.  
        
        
        %To output $h^*$ and $h^*_\sig$ such that $h^* \neq \PRF(\addsk^{\provider}||h^*_\sig)$, $\adv$ makes use of a zero-knowledge extractor $\zkExt$ to obtain a witness $w$ from $\pi_\own^*$. If $\pi_\own^*$ is valid, $w$ will also be valid. Now we show that $w$ is valid only with a negligible probability due to the following reasons -- i) Since $\sn^*=\sn$ where $\sn$ is part of $\tx \in \ledger$, the extractor finds a collision for $\PRF$ used to generate $\sn$ which is required to be collision-resistant, a contradiction. ii) If $w$ is valid, $h^*=\PRF(\addsk, h_\sig^*)$ but this contradicts the conditions of event $E_4$.
        
        %Suppose $\tx^* = \tx$ except $\sigma^* \neq \sigma$.  This is similar to the case when $\tx^*$ is a store transaction, if $\pk_\sig^*=\pk_\sig$, $\adv$ can create a valid $\tx^*$ only by forging $\sigma^*$ such that $\signature.\Verify(\pk_\sig^*,m^*,\sigma^*)=1$ where $m^*=x^*||\pi_\own^*$. However, due to the SUF-CMA property of the signature scheme, this can only occur with negligible probability.
        
        
    %     \item Suppose $\tx^* = \tx$ except $\sigma^* \neq \sigma$ and $\pk_\sig^* \neq \pk_\sig $. Now, assume that adversary provides $\pi_\own^* = \pi_\own$. In order for $\zkVerify(\pp,x^*,\pi_\own^*)=1$ specifically, to bypass the statement verification $h^*=\PRF(\addsk^\provider||h_\sig^*)$, $\adv$~needs to provide $h^*_\sig = h_\sig$, where $h_\sig =H(\pk_\sig) $ and $h^*_\sig =H(\pk^*_\sig)$. This means that the adversary must find $\pk_\sig^*$ such that $H(\pk_\sig^*) = H(\pk_\sig)$ and $\pk_\sig^* \neq \pk_\sig $, which happens only with a negligible probability due to the collision-resistant property of the hash function $H$.
    %     \
    %     \item Suppose $\tx^*=\tx$ except $\sigma^* \neq \sigma, \pk_\sig^* \neq \pk_\sig $ and $\pi_\own^* \ne \pi_\own$. There are two possibilities that the adversary can win: \\
    %     1) $\adv$ produces a valid proof $\pi_\own^*$ to demonstrate $h^*=  \PRF(\addsk^{\provider}||h^*_\sig)$  for an arbitrary $h^*_\sig \ne h_\sig $. This requires knowledge of $\addsk^{\provider}$; however, due to the zero-knowledge property of the underlying proof system, the probability that $\adv$ can extract $\addsk^{\provider}$ from the previous proofs $\pi$ in the query phase is negligible.  
        
    %   2) $\adv$ produces an arbitrary proof $\pi_\own^*$ that convinces the verifier to accept $h^*=  \PRF(\addsk^{\provider}||h^*_\sig)$ for arbitrary $h^*_\sig \ne h_\sig $, without knowing the witness  $\addsk^{\provider}$. The soundness property of the underlying proof system implies that to produce a valid proof, the adversary must demonstrate the knowledge of $\addsk^{\provider}$. Therefore, the probability that the adversary can produce an arbitrary proof that convinces the verifier to accept, without knowing $\addsk^{\provider}$, is negligible.
       
       %the probability that the adversary can produce such an arbitrary proof
       
       %$\adv$ has to create a valid $\pi$ without knowledge of a witness, in particular,. Due to the zero-knowledge property of the underlying proof system, $\adv$ can create such a valid proof only with negligible probability. 
        %\\
        %2) $h^* \neq \PRF(\addsk^{\provider}||h^*_\sig)-$ In order to create a valid proof, $\adv$ uses an extractor $\ext$ to obtain a valid witness. However, due to the soundness property of the underlying proof system, such an extractor exists with a negligible probability. 
        
        %as a sub-routine and define an extractor $\ext$ which can extract valid witnesses, $w$, from a given $\pi$ such that $\zkVerify(\pp,x,\pi)=1$. $\advb$ first invokes $\adv$ to get $\tx^*$, then uses $\ext$ to obtain a valid $w^*$ for $\pi_\own^*$. Since $w^*$ is a valid witness, 
        
        
        % \item Suppose $\tx^*=\tx$ except $\pi_\own^* \ne \pi_\own$
        
        % \item $\sn^* \neq \PRF({\addsk^\provider}||\rho^*)-$
        % According to condition iii) $\sn^*$ is already revealed in $\tx$ which means that $\adv$ found a collision for $\PRF$ \thang{this is not correct. You need to think as adversary and start with the viewpoint of adversary first. (take a look at the above sample I wrote) Also, this analysis is about the uniqueness of sn. For example, why you dont permit the adv to use the same sn? }. Therefore, this condition occurs with a negligible probability. 
        % \\
        % Note that the case $\sn^* = \PRF({\addsk^\provider}||\rho^*)$ cannot occur as $\adv$ has no knowledge of $\addsk^\provider$
    \end{itemize}
    
       \textbf{Case 2.} We assume that $\adv$ creates store operation record, however, the same proof applies if $\adv$ creates share or assign operation records as well. Let $Q_\CreateAddress = \{1^\lambda, 1^\lambda, \dotsc\}$ be the queries by $\adv$ to $\CreateAddress$ and $R_\CreateAddress = \{(\addpk^{\owner,1}, \addsk^{\owner,1}), (\addpk^{\owner,2}, \addsk^{\owner,2}), \dotsc\}$ be the response from $\chal$. 
    \sloppy $Q_\Store=\{(\pp,D_1,\addsk^{\owner,1},\addpk^{\provider,1}), (\pp,D_2,\addsk^{\owner,2},\addpk^{\provider,2}), \dotsc\}$ be the queries created by $\adv$ and $R_\Store=\{(\tokenstore^1, \tx_\store^1), (\tokenstore^2, \tx_\store^2), \dotsc\}$ be the response by $\chal$. $\adv$ wins $\trnm_\Pi$ when it outputs a record $ \tx_\store^* $ such that (i) $m^* \neq m$, where $m$ is a part of $\tx_\store \in R$;  (ii) $ \Verify(\pp,\tx_\store^*,\set{L}') = 1 $, where $ \set{L}' $ is the state of the audit log preceding $\tx_\store$.

   We assume that $\adv$ successfully creates a store record $\tx_\store^*=(\sigpk^*, \sigma^*, \cm_\store^*, \h^*, \pi_\store^*, \tokenstore^*)$ with proof instance $ x^* = (\cm_\store^*, h^*)$ and $m^* = x^*||\pi_\store^*||\tokenstore^*$. 
    
    
    Let $E_1$ be the event that $\adv$ wins and there exists $\pk_\sig \in R_\Store$ such that $\pk_\sig^* = \pk_\sig$. %\thang{same pk, but at least one in the signature message should be different}
    
    $E_2:$ $\adv$ wins, $E_1$ does not occur, and there exist $\pk_\sig \in R_\Store$ such that $h^*_\sig = h_\sig$. %\thang {new $\pk_\sig$, all others do not matter}
    
    $E_3:$ $\adv$ wins, $(E_1, E_2)$ do not occur and  $h^* = \PRF(\addsk^{\owner^*}, h^*_\sig)$ for some $\addsk^{\owner^*} \in R_\CreateAddress$. %\thang{you need to define Q to store address created by Adv} %\thang{new $h^*$, new pk without CRH with any existing pk, but there is link between them in terms of PRF}.
    
%    $\adv$ wins if each of the following hold independently-
    Each of the above event captures all the possible modifications $\adv$ makes to $\tx_\store$ to obtain $\tx_\store^*$ such that $m^* \neq m$.
    %
    $E_1$ captures when $m^* \neq m$ but $\pk_\sig^* = \pk_\sig$.
    %
    $E_2$ captures when $m^* \neq m$ but $ \h_\sig^* = \h_\sig$.
    %
    $E_3$ captures when $m^* \neq m$ but $\h^* = \h$.
    %
    Note that we don't have $E_4$, like in \textbf{Case 1}, which captures $m^* \ne m$ and $\sn^* = \sn$ since the response to a query to one of the functions $\{\Store, \Share, \Access\}$ does not include $\sn$.
    
    Now we show that each event occurs with a neglible probability.
    \begin{itemize}
        \item We show that $\Pr[E_1] = \negl(\lambda) $. Let $\sigma^*$ be the signature in $\tx^*$ and $\sigma$ be signature in $\tx$ that has $\pk_\sig$. Because  $\pk_\sig = \pk^*_\sig$, both $\sigma^*$ and $\sigma$ are the signatures created from the same public key. Since $\adv$ wins, by definition, there exists $\tx_\store \in R_\Store $ such that $\m^* \ne \m$. To craft $m^* \ne m$, $\adv$ needs to produce $\sigma^*$ such that $\Sigma.\Verify(\pk_\sig^*, m^*, \sigma^*) = 1$, $m^* \ne m$ and $\pk_\sig = \pk_\sig^*$. However, this happens with negligible probability as it breaks the SUF-CMA property of the underlying signature scheme.
        
        \item We show that $\Pr[E_2] = \negl(\lambda) $.
        The proof outline follows the same as that shown for $E_2$ in \textbf{Case 1}. Basically, we show that the $\adv$ will have to find a collision of a hash function to win this event. However, this only occurs with negligible probability. 
        
        \item We show that $\Pr[E_3] = \negl(\lambda) $. Similar to how we prove $E_3$ occurs with negligible probability in \textbf{Case 1}, we construct an attacker $\advb$ that uses $\adv$ as a subroutine. The attacker is constructed such that it distinguishes between a $\PRF$ function and a random function with an overwhelming probability. However, due to the indistinguishability property of the $\PRF$ function, this happens with a negligible probability.  
    \end{itemize}
\end{proof}

\begin{Theorem}
	 \sys~satisfies audit log indistinguishability by \autoref{lind}
\end{Theorem}




% \thang{\textit{Proof Overview.} We show $\sys$ achieves audit log indistinguishability by defining an adversary who can issue records of any type. The record is sent to a challenger who does the verification before appending to the audit log.

% We define a set of ``games" where the challenger modifies one part of the record and show that the modification provides no added advantage to the adversary to distinguish between the records issued by him. This means that the audit log is indistinguishable. Finally, we show that the modifications we suggest is computationally equivalent to the original experiment, hence proving audit log indistinguishability of the original experiment.
% }
\begin{proof}

We show that the adversary cannot be able to infer any information on the audit log record in \sys~with high probability.
%
We define a sequence of hybrid games and show that they are indistinguishable.
%
We first define a simulation $\lind_\Sim$ of $\lind_\Pi$ that the challenger $\chal$ can execute to answer the adversary's queries $(Q,Q')$ as specified in \autoref{lind} as follows.

%We deduce the proof by showing that the queries ($Q, Q'$) answered by the challenger $\chal$ is independent of bit $b$. $\chal$ creates a simulation by performing the following modifications to the original functions before answering the queries ($Q, Q'$) --
\noindent \underline{The simulation $\lind_\Sim$:}
\begin{itemize}	
    \item To answer $\AssignOwner$ queries, $\chal$ modifies $\AssignOwner$ to create $\sn$ and $h$ randomly. $\cm_\own \gets \Com_{r_2}(k_2, \pp)$ is computed using random inputs $k_2, r_2$. The encrypted token $\tokenowner^*\gets\Enc(e_1,p_1)$ is generated using a random plaintext $p_1$ and key $e_1$. Finally, the proof $\pi_\own^* \gets \zkSim( x, \pp)$ is computed using a simulator.  
    \item To answer $\Share$ queries, $\chal$ replaces $h$ with a random value. The commitment is created as $\cm_\share^* \gets \Com_{r_3}(k_3, \pp)$ where $k_3, r_3$ are random inputs. $\tokenshare^*$ is created using a random plaintext $p_2$ and key $e_2$. Lastly, $\pi_\share^*$ is generated similar to how $\pi_\own^*$ is generated.
    \item To answer $\Access$ queries, $\chal$ replaces $h$ with a random value. $\chal$ creates $\cm_\access^* \gets \Com_{r_4}(k_4, \pp)$ where $k_4, r_4$ are random inputs and creates $\tokenaccess^*$ using a random plaintext $p_3$ and key $e_3$. Finally, $\pi_\access^*$ is generated in a similar fashion as $\pi_\own^*$.
\end{itemize}

In all the above cases, the simulated functions compute $Q$ and $Q'$ independent of bit $b$ -
\[
\Pr[b=b'] = \frac{1}{2}
\]

Therefore, $\adv$ has negligible advantage in $\lind_\Sim$. 

Now, to show that $\lind_\Sim$ is indistinguishable from $\lind_\Pi$, we define a sequence of hybrid games as follows --

\begin{itemize}
    \item $G_0$ -- This is the original protocol, where the challenger $\chal$ executes protocols in \autoref{ch:method} to answer $\adv$ queries. 
    
    \item $G_1$ -- $G_1$ is the same as $G_0$, except that to answer queries from $\adv$, $\chal$ uses a zero-knowledge simulator to generate a proof $\pi^* = \zkSim(\pp, x)$ with an arbitrary witness. Due to the zero-knowledge property of the underlying proof system, we say that $\lind_1$ is indistinguishable from $\lind_0$.
    
    \item $G_2$ -- $G_2$ is same as $G_1$ except that $\chal$ generates the encrypted tokens differently to answer queries from $\adv$. In particular, $\chal$ generates $\tokenstore^*, \tokenowner^*, \tokenshare^*, \tokenaccess^*$ (depending on the query) using $\Enc(e,p)$ where $p$ is a random plaintext and $e$ is a random public encryption key. Due to the IND-CCA property of the underlying encryption scheme, $\adv$ cannot distinguish between a ciphertext generated from a random plaintext or a particular plaintext. Also, due to the IK-CCA property, $\adv$ cannot distinguish between a ciphertext generated from a random public key or a particular public key. Due to the IK-CCA and IND-CCA property of the underlying encryption scheme, $G_2$ is indistinguishable from $G_1$.
    
    \item $G_3$ -- $G_3$ is the same as $G_2$, however, $\chal$ substitutes $\PRF$ generated values with random strings to answer queries from $\adv$. Due to the indistinguishability property of the $\PRF$ function from a random function, this modification gives no added advantage to $\adv$. Therefore, $G_3$ is indistinguishable from $G_2$.
    
    \item $G_4$ -- $G_4$, equivalent to simulation $\lind_\Sim$, is identical to $G_3$ except that $\chal$ computes $\cm_\store^*, \cm_\own^*, \cm_\share^*, \cm_\access^*$ (depending on the query) as $\Com_r(k, \pp)$ where $r$ and $k$ are random inputs. Due to the hiding property of the underlying commitment scheme, $G_4$ is indistinguishable from $G_3$. Note that all modifications are independent of bit $b$.
\end{itemize}

We can see that $\lind_\Pi = G_0 \stackrel{c}{\approx} G_1 \stackrel{c}{\approx} G_2 \stackrel{c}{\approx}  G_3 \stackrel{c}{\approx} G_4 = \lind_\Sim$ and this completes the indistinguishability proof.
\end{proof}

==> security_og.tex <==
\section{Security Analysis}
\begin{Theorem}
    \sys~satisfies record non-malleability by \autoref{lnm}.
\end{Theorem}
\begin{proof}  Let $Q_\CreateAddress = \{1^\lambda, 1^\lambda, \dotsc\}$ be the queries by $\adv$ to $\CreateAddress$ and $R_\CreateAddress = \{(\addpk^{\provider,1}, \addsk^{\provider,1}), (\addpk^{\provider,2}, \addsk^{\provider,2}), \dotsc\}$ be $\chal$'s response. 

Without loss of generality, let
    \sloppy $Q_\AssignOwner=\{(\tokenstore^1,\addsk^{\provider,1},\addpk^{\owner,1},\pp), (\tokenstore^2,\addsk^{\provider,2},\addpk^{\owner,2},\pp),, \dotsc\}$ be the queries created by $\adv$ and $R_\AssignOwner=\{(\tokenowner^1, \tx_\own^1), (\tokenowner^2, \tx_\own^2), \dotsc\}$ be the response by $\chal$. $\adv$ wins the experiment $\trnm$ when it outputs a record $ \tx_\own^* $ such that (i) $m^* \neq m$, where $m$ is the message in some $\tx_\own \in R_\AssignOwner$;  (ii) $ \mathsf{VerifyLog}(\tx_\own^*,\set{L}',\pp) = 1 $, where $ \set{L}' $ is the state of the audit log preceding $\tx_\own$; (iii) $\sn^*=\sn$ iff $\tx^*$ is an ownership record.

  Assume that  $\adv$ wins by creating a record $\tx_\own^*=(\rt_\store^*, \sigpk^*, \sigma^*,  \sn^*, \cm_\own^*, \h^*, \pi_\own^*, \tokenowner^*)$ with proof instance $ x^* = (\rt_\store^*, \sn^*, \cm_\own^*, h^*)$ and $m^* = x^*||h_\sig^*||\pi_\own^*||\tokenowner^*$. We consider the following events.
    
    
    $E_1:$ $\adv$ wins, and there exists $\pk_\sig \in R_\AssignOwner$ such that $\pk_\sig^* = \pk_\sig$. To win, $\adv$ produces $\sigma^*$ such that $\Sigma.\Verify(\pk_\sig^*, m^*, \sigma^*) = 1$, $m^* \ne m$ and $\pk_\sig^* = \pk_\sig$. However, due to the SUF-CMA property of the signature scheme \cite{schnorr}, this happens with negligible probability.  %\thang{same pk, but at least one in the signature message should be different}
    
    $E_2:$ $\adv$ wins, $E_1$ does not occur, and there exists $\pk_\sig \in R_\AssignOwner$ such that $h^*_\sig = h_\sig$. When $\adv$ wins, it crafts a $h^*_\sig = h_\sig$ when $\pk_\sig^* \ne \pk_\sig$. Due to the collision-resistant property of the hash function \cite{mimc}, this occurs with negligible probability. %\thang {new $\pk_\sig$, all others do not matter}
    
    $E_3:$ $\adv$ wins, $(E_1, E_2)$ do not occur and  $h^* = \PRF(\addsk^{\provider^*}|| h^*_\sig)$ for some $\addsk^{\provider^*} \in R_\CreateAddress$. Due to the one-wayness property of $\PRF$ (used to generate $\addpk^{\provider^*}$), $\adv$ will not be able to deduce $\addsk^{\provider^*}$ and generates $h^*$ with a random key. However, due to indistinguishability property of $\PRF$ (used to generate $h^*$), $\adv$ wins negligbly.
    
    $E_4:$ $\adv$ wins, $(E_1, E_2, E_3)$ do not occur, $\tx^*$ is  an ownership record and  $h^* \ne \PRF(\addsk^{\provider^*}|| h^*_\sig)$ for \textit{all} $\addsk^{\provider^*} \in R_\CreateAddress$. If $\adv$ wins, it outputs a modified record such that $\sn^*=\sn$. However, since in $E_4$ $\addsk^{\provider^*} \ne \addsk^{\provider}$, it means that to generate $\sn^*$, $\adv$ found a collision in the $\PRF$ needed to generate $\sn$ which occurs with negligible probability due to the collision-resistant property of the $\PRF$ function used to generate $\sn$. %\thang{completely new $h^*$, $pk^*$}
    \qedhere
%    $\adv$ wins if each of the following hold independently-
    % Each of the above event captures all the possible modifications $\adv$ makes to $\tx_\own$ to obtain $\tx_\own^*$ such that $\tx_\own^* \neq \tx_\own$.
    % %
    % $E_1$ captures when $\tx_\own^* \neq \tx_\own$ but $\pk_\sig^* = \pk_\sig$.
    % %
    % $E_2$ captures when $\tx_\own^* \neq \tx_\own$ but $ \h_\sig^* = \h_\sig$.
    % %
    % $E_3$ captures when $\tx_\own^* \neq \tx_\own$ but $\h^* = \h$.
    % %
    % $E_4$ captures when $\tx_\own^* \neq \tx_\own$. 
    % %
    % Note that in every event $\sn^* = \sn$ as it is a condition imposed by the game. 
    
    % Now we present the intuition to show that each event occurs with negligible probability.
    
    % $E_1$ occurs iff $\adv$ can forge a new signature $\sigma^*$ in $\tx^*$ for the message $m^*$ that contain a new serial number $\sn^*$, under the same signing and verification key, which only happens with negligible probability due to the SUF-CMA property of signature scheme.
    
    % $E_2$ only occurs iff  $\adv$ can provide a new $\pk^*_\sig$ in $\tx^*$ such that $\CRH(\pk^*_\sig) = \CRH(\pk_\sig)$, which only happens with negligible probability due to the collision-resistant property of $H$
    
    % $E_3$ occurs iff $\adv$ can distinguish $\PRF$ from a random function, which happens with negligible probability.
    
    % $E_4$ occurs iff $\adv$ can find a collision for the $\PRF$ used to generate $\sn$, which happens only with negligible probability.
    
    % \begin{itemize}
        % \item We show that $\Pr[E_3] = \negl(\lambda) $ by contradiction. Assume $\epsilon = \Pr[E_3]$ is non negligible. Now we construct an attacker $\advb$ that distinguishes with a non negligible probability a pseudorandom function $\PRF$ from a random function $\RAND$ by crafting $\tx^\dagger_\own $. $\advb$ follows the same conditions that $\adv$ follows to craft $\tx^*$. To do so, $\advb$ selects a random $(\addpk^{\provider^\dagger}, \addsk^{\provider^\dagger}) \in R_\CreateAddress$. Then, $\advb$ crafts $h^\dagger = \owner^\PRF(\addsk^{\provider^\dagger}||h_\sig^\dagger)$ or $\h^\dagger = \owner^\RAND(\addsk^{\provider^\dagger}||h_\sig^\dagger)$ using either of the two oracles $\owner^\PRF$ or $\owner^\RAND$.
        % $\advb$ then invokes $\adv$ which outputs $\tx_\own^*$. Now, according to conditions of $E_3$, $\advb$ outputs 1 (i.e, wins) iff $h^\dagger = \h^*$ where $h^*$ is a part of $\tx_\own^*$ crafted by $\adv$. 
        % $\advb$ \textit{aborts and wins} if it outputs $\h^\dagger = \h^*$ \textit{before} $\adv$ outputs $\tx_\own^*$. 
        
        % Now, we calculate the probability that $\advb$ wins. Note that $\advb$ wins when it aborts \textit{or} if it outputs 1 and does not abort.  Recall that $\advb$ aborts iff it outputs $\h^\dagger = \h^*$ before $\adv$ outputs a $\h^*$. Then, when $\adv$ finally outputs $h^*$, it would imply that $\pk_\sig^* = \pk_\sig^\dagger$ and $\h_\sig^* = \h_\sig^\dagger$ which does not hold in $E_3$ (when $E_3$ occurs, $E_1$ and $E_2$ don't occur). Hence, $\advb$ aborts with negligible probability. Therefore, to calculate the probability with which $\advb$ wins, it is sufficient to calculate the probability that $\advb$ outputs 1 and does not abort.
        
        % Since $\advb$ uses either of the two oracles, we have the following cases -- i) $\h^\dagger$ is created using $\owner^\RAND$.
        % If $h^\dagger$ is of one bit length, the probability that $\advb$ wins and does not abort is $\frac{1}{2}$. Since the output is of length $\lvert \h^\dagger \rvert$, the probability that $\advb$ wins and does not abort is ($\frac{1}{2})^{\lvert \h^\dagger \rvert}$, which is negligible. 
        
        % ii) $\h^\dagger$ is crafted using $\owner^\PRF$.
        % Since $\adv$ performs the experiment independent of $\addsk^{\provider^\dagger}$, probability that $\addsk^{\provider^*} = \addsk^{\provider^\dagger}$ will be $\frac{1}{\lvert R_\CreateAddress \rvert}$. Therefore, the probability that $\advb$ wins and $\advb$ does not aborts is at least $\frac{\epsilon}{\lvert R_\CreateAddress \rvert}$. Since $\epsilon$ is non negligible (by assumption), $\frac{\epsilon}{\lvert R_\CreateAddress \rvert}$ is also non negligible.
        
        % Now to calculate the probability that $\advb$ distinguishes between a pseudorandom and a random function, we find the difference in probabilities when $\advb$ wins using $\owner^\PRF$ and $\owner^\RAND$. Using $\owner^\RAND$, $\advb$ wins with a non negligible probability as $\adv$ will be using random guesses. Using $\owner^\PRF$, $\advb$ wins with a non negligible probability $\frac{\epsilon}{|R_\CreateAddress|}$ as $\epsilon$ was assumed to be non negligible. Therefore, the difference is non negligible, a contradiction. 
        
        
        % \item We show that $\Pr[E_4] = \negl(\lambda) $ by contradiction.  We craft an algorithm $\advb$ which finds collisions in $\PRF$ used to compute $\sn$ with an overwhelming probability. $\advb$ first runs $\adv$ to obtain $\tx_\own^*$. Then, it runs a zero-knowledge extractor $\zkExt$ to obtain a witness $w$. If $w$ is invalid, $\adv$ aborts and returns 0. If $w$ is valid, find $\tx \in R_\AssignOwner$ with $\sn^* = \sn$. If $\addsk^{\provider^*} \ne \addsk^{\provider}$ and $\sn^* = \sn$, $\advb$ found a collision for $\PRF$. 
        
        % Now we show that $\addsk^{\provider^*} \ne \addsk^{\provider}$ occurs with overwhelming probability. Since $w$ is valid, $\h^* = \PRF(\addsk^{\provider^*}||h_\sig^*)$. Now, if $\addsk^{\provider^*} = \addsk^\provider$, it contradicts conditions of $E_4$. Therefore, if $E_4$ occurs, $\addsk^{\provider^*} \neq \addsk^\provider$ with overwhelming probability. This implies that $\advb$ always finds a $\tx \in R_\AssignOwner$ such that $\sn^* = \sn$ with an overwhelming probability, a contradiction.
        
        
        %To output $h^*$ and $h^*_\sig$ such that $h^* \neq \PRF(\addsk^{\provider}||h^*_\sig)$, $\adv$ makes use of a zero-knowledge extractor $\zkExt$ to obtain a witness $w$ from $\pi_\own^*$. If $\pi_\own^*$ is valid, $w$ will also be valid. Now we show that $w$ is valid only with a negligible probability due to the following reasons -- i) Since $\sn^*=\sn$ where $\sn$ is part of $\tx \in \ledger$, the extractor finds a collision for $\PRF$ used to generate $\sn$ which is required to be collision-resistant, a contradiction. ii) If $w$ is valid, $h^*=\PRF(\addsk, h_\sig^*)$ but this contradicts the conditions of event $E_4$.
        
        %Suppose $\tx^* = \tx$ except $\sigma^* \neq \sigma$.  This is similar to the case when $\tx^*$ is a store transaction, if $\pk_\sig^*=\pk_\sig$, $\adv$ can create a valid $\tx^*$ only by forging $\sigma^*$ such that $\signature.\Verify(\pk_\sig^*,m^*,\sigma^*)=1$ where $m^*=x^*||\pi_\own^*$. However, due to the SUF-CMA property of the signature scheme, this can only occur with negligible probability.
        
        
    %     \item Suppose $\tx^* = \tx$ except $\sigma^* \neq \sigma$ and $\pk_\sig^* \neq \pk_\sig $. Now, assume that adversary provides $\pi_\own^* = \pi_\own$. In order for $\zkVerify(\pp,x^*,\pi_\own^*)=1$ specifically, to bypass the statement verification $h^*=\PRF(\addsk^\provider||h_\sig^*)$, $\adv$~needs to provide $h^*_\sig = h_\sig$, where $h_\sig =H(\pk_\sig) $ and $h^*_\sig =H(\pk^*_\sig)$. This means that the adversary must find $\pk_\sig^*$ such that $H(\pk_\sig^*) = H(\pk_\sig)$ and $\pk_\sig^* \neq \pk_\sig $, which happens only with a negligible probability due to the collision-resistant property of the hash function $H$.
    %     \
    %     \item Suppose $\tx^*=\tx$ except $\sigma^* \neq \sigma, \pk_\sig^* \neq \pk_\sig $ and $\pi_\own^* \ne \pi_\own$. There are two possibilities that the adversary can win: \\
    %     1) $\adv$ produces a valid proof $\pi_\own^*$ to demonstrate $h^*=  \PRF(\addsk^{\provider}||h^*_\sig)$  for an arbitrary $h^*_\sig \ne h_\sig $. This requires knowledge of $\addsk^{\provider}$; however, due to the zero-knowledge property of the underlying proof system, the probability that $\adv$ can extract $\addsk^{\provider}$ from the previous proofs $\pi$ in the query phase is negligible.  
        
    %   2) $\adv$ produces an arbitrary proof $\pi_\own^*$ that convinces the verifier to accept $h^*=  \PRF(\addsk^{\provider}||h^*_\sig)$ for arbitrary $h^*_\sig \ne h_\sig $, without knowing the witness  $\addsk^{\provider}$. The soundness property of the underlying proof system implies that to produce a valid proof, the adversary must demonstrate the knowledge of $\addsk^{\provider}$. Therefore, the probability that the adversary can produce an arbitrary proof that convinces the verifier to accept, without knowing $\addsk^{\provider}$, is negligible.
       
       %the probability that the adversary can produce such an arbitrary proof
       
       %$\adv$ has to create a valid $\pi$ without knowledge of a witness, in particular,. Due to the zero-knowledge property of the underlying proof system, $\adv$ can create such a valid proof only with negligible probability. 
        %\\
        %2) $h^* \neq \PRF(\addsk^{\provider}||h^*_\sig)-$ In order to create a valid proof, $\adv$ uses an extractor $\ext$ to obtain a valid witness. However, due to the soundness property of the underlying proof system, such an extractor exists with a negligible probability. 
        
        %as a sub-routine and define an extractor $\ext$ which can extract valid witnesses, $w$, from a given $\pi$ such that $\zkVerify(\pp,x,\pi)=1$. $\advb$ first invokes $\adv$ to get $\tx^*$, then uses $\ext$ to obtain a valid $w^*$ for $\pi_\own^*$. Since $w^*$ is a valid witness, 
        
        
        % \item Suppose $\tx^*=\tx$ except $\pi_\own^* \ne \pi_\own$
        
        % \item $\sn^* \neq \PRF({\addsk^\provider}||\rho^*)-$
        % According to condition iii) $\sn^*$ is already revealed in $\tx$ which means that $\adv$ found a collision for $\PRF$ \thang{this is not correct. You need to think as adversary and start with the viewpoint of adversary first. (take a look at the above sample I wrote) Also, this analysis is about the uniqueness of sn. For example, why you dont permit the adv to use the same sn? }. Therefore, this condition occurs with a negligible probability. 
        % \\
        % Note that the case $\sn^* = \PRF({\addsk^\provider}||\rho^*)$ cannot occur as $\adv$ has no knowledge of $\addsk^\provider$
    % \end{itemize}
    

%       We assume that $\adv$ modifies a response to a $\Store$ request, however, the same proof applies if $\adv$ modifies either $\Share$ or $\Access$ response as well. Let $Q_\CreateAddress = \{1^\lambda, 1^\lambda, \dotsc\}$ be the queries by $\adv$ to $\CreateAddress$ and $R_\CreateAddress = \{(\addpk^{\owner,1}, \addsk^{\owner,1}), (\addpk^{\owner,2}, \addsk^{\owner,2}), \dotsc\}$ be the response from $\chal$. 
%     \sloppy $Q_\Store=\{(\pp,D^1,\addsk^{\owner,1},\addpk^{\provider,1}), (\pp,D^2,\addsk^{\owner,2},\addpk^{\provider,2}), \dotsc\}$ be the queries created by $\adv$ and $R_\Store=\{(\tokenstore^1, \tx_\store^1), (\tokenstore^2, \tx_\store^2), \dotsc\}$ be the response by $\chal$. $\adv$ wins the Record-Entry Non-Malleability game when it outputs a record $ \tx_\store^* $ such that (i) $m^* \neq m$, where $m$ is a part of $\tx_\store \in R$;  (ii) $ \mathsf{VerifyLog}(\pp,\tx_\store^*,\set{L}') = 1 $, where $ \set{L}' $ is the state of the audit log preceding $\tx_\store$.

%   We assume that $\adv$ successfully creates a store record $\tx_\store^*=(\sigpk^*, \sigma^*, \cm_\store^*, \h^*, \pi_\store^*, \tokenstore^*)$ with proof instance $ x^* = (\cm_\store^*, h^*)$ and $m^* = x^*||\pi_\store^*||\tokenstore^*$. 
    
    
%     Let $E_1$ be the event that $\adv$ wins and there exists $\pk_\sig \in R_\Store$ such that $\pk_\sig^* = \pk_\sig$. %\thang{same pk, but at least one in the signature message should be different}
    
%     $E_2:$ $\adv$ wins, $E_1$ does not occur, and there exist $\pk_\sig \in R_\Store$ such that $h^*_\sig = h_\sig$. %\thang {new $\pk_\sig$, all others do not matter}
    
%     $E_3:$ $\adv$ wins, $(E_1, E_2)$ do not occur and  $h^* = \PRF(\addsk^{\owner^*}, h^*_\sig)$ for some $\addsk^{\owner^*} \in R_\CreateAddress$. %\thang{you need to define Q to store address created by Adv} %\thang{new $h^*$, new pk without CRH with any existing pk, but there is link between them in terms of PRF}.
    
% %    $\adv$ wins if each of the following hold independently-
%     % Each of the above event captures all the possible modifications $\adv$ makes to $\tx_\store$ to obtain $\tx_\store^*$ such that $m^* \neq m$.
%     % %
%     % $E_1$ captures when $m^* \neq m$ but $\pk_\sig^* = \pk_\sig$.
%     % %
%     % $E_2$ captures when $m^* \neq m$ but $ \h_\sig^* = \h_\sig$.
%     % %
%     % $E_3$ captures when $m^* \neq m$ but $\h^* = \h$.
%     % %
%     Note that we don't have $E_4$, like in \textbf{Case 1}, which captures $\tx^* \ne \tx$ and $\sn^* = \sn$ since the response to a query to one of the functions $\{\Store, \Share, \Access\}$ does not include $\sn$.
    
%     Now we show that each event occurs with a neglible probability.
%     \begin{itemize}
%         \item We show that $\Pr[E_2] = \negl(\lambda) $. Since $\adv$ wins, by definition, there exists $\tx_\store \in R_\Store $ such that $\m^* \ne \m$. To craft $m^* \ne m$, $\adv$ needs to produce $\sigma^*$ such that $\Sigma.\Verify(\pk_\sig^*, m^*, \sigma^*) = 1$, $m^* \ne m$ and $\pk_\sig = \pk_\sig^*$. However, this happens with negligible probability as it breaks the SUF-CMA property of the underlying signature scheme.
        
%         \item We show that $\Pr[E_2] = \negl(\lambda) $ and $\Pr[E_3] = \negl(\lambda) $ similar to how we prove $E_2, E_3$ occurs with negligible probability in \textbf{Case 1}. 
%     \end{itemize}
\end{proof}

\begin{Theorem}
	 \sys~satisfies audit log indistinguishability by \autoref{lind}
\end{Theorem}
% \begin{proof}
% We deduce the proof by showing that the queries ($Q, Q'$) answered by the challenger $\chal$ is independent of bit $b$. $\chal$ creates a simulation $\lind_\Sim$ of $\lind_\Pi$ by performing modifications to the original functions before answering the queries ($Q, Q'$). 
% %
% $\chal$ modifies the commitment in the response to use a $\cm^* = \Com_{r}(k)$ by using random inputs $k, r$. 
% %
% Due to the hiding property of the commitment scheme, this modification is computationally indistinguishable from the original experiment.
% %
% Next, $\chal$ replaces the token in the response with a $\token^*=\encryption.\Enc(e, p)$ where $e$ is a random public key and $p$ is a random plaintext.
% %
% Due to the IK-CCA and IND-CCA properties of the generated ciphertext, this modification is computationally indistinguishable from the original experiment.
% %
% $\chal$ replaces all $\PRF$ generated values (i.e, $h, \sn$) in the response with values generated using a random function.
% %
% This modification is computationally indistinguishable from the original experiment due to the indistinguishability property of $\PRF$.
% %
% Finally, the zero-knowledge proof in the response are replaced by a simulated proof created $\pi^* = \zkSim(\pp, x, w^*)$ with an arbitrary witness $w^*$.
% %
% Due to the zero-knowledge property of the proof, this modification is computationally indistinguishable from the original experiment.


% Note, in $\lind_\Sim$, the functions compute $Q$ and $Q'$ independent of bit $b$. Therefore, $\adv$ wins $\lind_\Sim$ with negligible probability $\Pr[b=b'] = \frac{1}{2}$.
% %
% Since $\lind_\Sim$ is indistinguishable from the original experiment $\lind_\Pi$, $\adv$ wins $\lind_\Pi$ negligibly.
% %

% \qedhere
% \end{proof}
\begin{proof}
	$\chal$ creates a simulation $\lind_\Sim$ that can answer the queries ($Q, Q'$) independent to the selected bit $ b $ as follows. $\chal$ modifies the commitment $\cm_\store^* \gets \Com_{r}(k,\pp)$ by using random inputs $k, r$. To answer $\AssignOwner$ queries, $\chal$ modifies $\AssignOwner$ to create $\sn$ and $h$ randomly. $\cm_\own$ is computed like in $\Store$. $\tokenowner^* \gets \encryption.\Enc(e,p)$ is generated using a random plaintext $p$ and key $e$. Proof $\pi_\own^* \gets \zkSim(x,\pp)$ is computed using a simulator. To answer $\Share$ or $\Access$ queries, $\chal$ computes $h$, commitments ($\cm_\share$/$\cm_\access$), tokens ($\tokenshare$/$\tokenaccess$), proofs ($\pi_\share$/$\pi_\access$) by following modifications in $\AssignOwner$. 

We prove this by constructing a sequence of hybrid games and show that they are indistinguishable as follows. 
%
Let $G_0$ be the original protocol $\lind_\Pi$. We define $G_1$ as similar to $G_0$, except that $\chal$ modifies the commitment in the response to use a $\cm^* \gets  \Com_{r}(k, \pp)$ by using random inputs $k, r$. We have that $ G_1 \stackrel{c}{\approx} G_0 $ due to  the hiding property of the commitment scheme.%
We define $G_2$ as similar  to $G_1$, except that the token in the response is replaced with $\token^* \gets \encryption.\Enc(e, p)$ where $e$ is a random public key and $p$ is a random plaintext.
%
We argue that $ G_2 \stackrel{c}{\approx} G_1 $ due to the IND-CCA and IK-CCA properties of the encryption scheme \cite{dhaes}.
%
We define $G_3$ as similar to $G_2$, except that all $\PRF$ generated values (i.e, $h, \sn$) in the response are replaced with values generated using a random function.
%
We say that $ G_3 \stackrel{c}{\approx} G_2 $ due to the  indistinguishability between $\PRF$ and random number function.
%
Finally, we define $ G_4 $ as similar to $G_3$, except that the zero-knowledge proof in the response is replaced by a simulated proof $\pi^* \gets \zkSim(x, \pp)$.
%
We have that $ G_4 \stackrel{c}{\approx} G_3 $ due to the zero-knowledge property of the proof system.


We can see that  $G_4$ is the simulation  $\lind_\Sim$. 
%
Therefore, $\lind_\Pi = G_0 \stackrel{c}{\approx} G_1 \stackrel{c}{\approx} G_2 \stackrel{c}{\approx} G_3 \stackrel{c}{\approx} G_4 = \lind_\Sim$.
Since $\lind_\Sim$ can simulate the response to $Q$ and $Q'$ independent of bit $b$, $\adv$ can win $\lind_\Pi$ game with negligible probability.
%
\qedhere
\end{proof}
